Minimax Optimality of the Probability Flow ODE for Diffusion Models

Score-based diffusion models have become a foundational paradigm for modern generative modeling, demonstrating exceptional capability in generating samples from complex high-dimensional distributions. Despite the dominant adoption of probability flow ODE-based samplers in practice due to their superior sampling efficiency and precision, rigorous statistical guarantees for these methods have remained elusive in the literature. This work develops the first end-to-end theoretical framework for deterministic ODE-based samplers that establishes near-minimax optimal guarantees under mild assumptions on target data distributions. Specifically, focusing on subgaussian distributions with $\beta$-H\"older smooth densities for $\beta\leq 2$, we propose a smooth regularized score estimator that simultaneously controls both the $L^2$ score error and the associated mean Jacobian error. Leveraging this estimator within a refined convergence analysis of the ODE-based sampling process, we demonstrate that the resulting sampler achieves the minimax rate in total variation distance, modulo logarithmic factors. Notably, our theory comprehensively accounts for all sources of error in the sampling process and does not require strong structural conditions such as density lower bounds or Lipschitz/smooth scores on target distributions, thereby covering a broad range of practical data distributions.

==> proof-thm.tex <==
%!TEX root = ODE-minimax.tex

\section{Proof of Theorems}\label{sec:proof_of_theorem}


For notational convenience, we define $g_t(x):\bR^d\to\bR^d$ as
\begin{align}\label{eq:g_t}
	g_t(x) \defn \frac1t\bE \big[(X_0-x)\vphi_t(X_0-x) \big].
	% = -\frac{1}{t}xp_{t}(x) + \frac1t\bE \big[ X_0\vphi_t(X_0-x) \big] 
\end{align}
and define $H_t(x):\bR^d\to\bR^{d\times d}$ as
\begin{align}\label{eq:Phi-def}
	H_t(x) & \defn \bE\big[\wh{H}_t(x)\big] = \frac1{t^2}\bE\big[(X_0-x)(X_0-x)^\top \vphi_t(X_0-x)\big].
\end{align}

Notice that
\begin{align*}
	\frac{g_t(x)}{p_{t}(x)} & = \frac1{t} \int_{y\in\bR^d} (y-x) \frac{1}{(2\pi t)^{d/2}}\exp\left(-\frac{\|y-x\|_2^2}{2t}\right) \frac{p_0(y)}{p_{t}(x)} \diff y \notag \\
	&  = \frac1{t} \int_{y\in\bR^d} (y-x) p_{X_0 \mid X_t}(y \mid x) \diff y \notag \\
	&  = \frac1{t} \bE\big[(X_0-x) \mid X_t = x\big] = s_{t}(x)
\end{align*}
where the second line holds as $X_t \mid X_0=y \sim \cN(y,tI_d)$. Similarly, one has
\begin{align}
	% \frac{\bE\big[\wh{H}_t(x)\big]}{\bE\big[\wh{p}_t(x)\big]} & = 
	\frac{H_t(x)}{p_{t}(x)} 
	& = \frac1{t^2} \int_{y\in\bR^d} (y-x)(y-x)^\top \frac{1}{(2\pi t)^{d/2}}\exp\left(-\frac{\|y-x\|_2^2}{2t}\right) \frac{p_0(y)}{p_{t}(x)} \diff y \notag \\
	&  = \frac1{t^2} \int_{y\in\bR^d} (y-x)(y-x)^\top p_{X_0 \mid X_t}(y \mid x) \diff y \notag \\
	&  = \frac1{t^2} \bE\big[(X_0-x)(X_0-x)^\top \mid X_t = x\big], \label{eq:Phi-p-exp}
\end{align}

Therefore, in light of the expression of the Jacobian $J_{s_{t}}(x)$ in \eqref{eq:Jacobian}, we can alternatively express it as
\begin{align}
	J_{s_{t}}(x) & = -\frac1t I_d + \frac{H_t(x)}{p_{t}(x)} - s_{t}(x)s_{t}(x)^\top\label{eq:Jacobian-expression}.
\end{align}



\begin{lemma}\label{lemma:MSE-density}
For any $x\in\bR^d$, one has
	\begin{align}
		\bE\Big[ \big|\wh{p}_t(x)-p_{t}(x)\big|^2 \Big] & 
	\leq \frac{p_{t}(x)}{n(2\pi t)^{d/2}} \label{eq:MSE-pdf};\\
	\bE\Big[ \big\| \wh{g}_t(x)-g_t(x)\big\|_2^2 \Big] & \leq \frac{p_{t}(x)}{n(2\pi t)^{d/2}t} \label{eq:MSE-g},\\
	\bE\Big[\big\|\wh{H}_t(x)-H_t(x)\big\|\Big] &\lesssim \frac1{n(2\pi t)^{d/2}t} + \frac1t\sqrt{\frac{p_{t}(x)}{n(2\pi t)^{d/2}}}
	 % \frac1{(2\pi)^{d/4}} \frac{\sqrt{p_{t}(x)}}{\sqrt{n}\,t^{d/4+1}}. 
	 \label{eq:Phi-error-exp-UB}
\end{align}

	Moreover, the event $\cE_t(x)$ defined in \eqref{eq:event-E} obeys
	\begin{align}
		\bP\big(\cE_t^\setc(x) \big) \lesssim n^{-10}. \label{eq:density-concen-ineq}
	\end{align}
\end{lemma}

\begin{proof}
	See Appendix~\ref{sub:proof_of_lemma_ref_lemma_mse-density}.
\end{proof}


\begin{lemma}\label{lemma:score-Jacobian-UB-prob-high}
	For any $x\in\cF_t$, one has
	\begin{subequations}\label{eq:score-Jacobian-UB-prob-high}
		\begin{align}
		\|s_{t}(x)\|_2 &\lesssim \sqrt{\frac{\log n}{t}} \label{eq:score-UB-prob-high},\\
		\big\|J_{s_{t}}(x)\big\| &\lesssim \frac{\log n}{t} \label{eq:Jacobian-UB-prob-high},\\
		\big\|H_t(x)\big\| &\lesssim \frac{p_{t}(x)\log n}{t}  \label{eq:Sigma-UB-prob-high}.
	\end{align}
	\end{subequations}
\end{lemma}

\begin{proof}
	See Appendix~\ref{sub:proof_of_lemma_ref_lemma_score_jacobian_ub_prob_high}.
\end{proof}


\begin{lemma}\label{lemma:high-density-set-bound}
For any $t \leq \ol T = n^{C_{T}}$ where $C_{T}$ is some absolute constant, one has
	\begin{align}
		|\cF_t| &\leq C_5 (t^{d/2} + \sigma^d)(\log n)^{d/2} \label{eq:high-density-set-UB}.
	\end{align}
where $C_5=C_5(d)>0$ is some constant that only depends on $d$. Further, for any $x\in\cF_t$, one has
\begin{align}
		\int_{\cF_t} \|s_{t}(x)\|_2^2 \diff x &\leq C_5 \frac{t^{d/2}+\sigma^d}{t^{d/2}} (\log n)^{d/2+1}. \label{eq:high-density-set-score-UB}
\end{align}
\end{lemma}

\begin{proof}
	See Appendix~\ref{sub:proof_of_lemma_ref_lemma_high_density_set_bound}.
\end{proof}



\subsection{Proof of Theorem~\ref{thm:score-error}}\label{sub:proof_of_lemma_ref_lemma_score-error}



Recall the definitions of $\cF_t$ and $\cE_t(x)$ in \eqref{eq:rho-t} and \eqref{eq:event-E}, respectively. 
%
For any $x\in\cF_t$, one has
\begin{align*}
	p_{t}(x) \geq \rho_t \defn  \frac{c_\rho\log n}{n(2\pi t)^{d/2}} \geq 2C_\cE \bigg( \frac{\log n}{n(2\pi t)^{d/2}}+ \sqrt{\frac{p_{t}(x)\log n}{n(2\pi t)^{d/2}}} \bigg),
\end{align*}
since we set $c_\rho = 4C_\cE \vee 2 \geq 2C_\cE(1+1/\sqrt{c_\rho})$.
%
Thus, on the event $\cE_t(x)$, one has
\begin{align}
	\wh p_{t}(x) & \geq p_{t}(x) - C_\cE \bigg( \frac{\log n}{n(2\pi t)^{d/2}}+ \sqrt{\frac{p_{t}(x)\log n}{n(2\pi t)^{d/2}}} \bigg)
	\geq \frac12 p_{t}(x) \geq \frac{\log n}{n(2\pi t)^{d/2}} = p_t^\thr \label{eq:p-hat-LB}.
\end{align}
where the last step holds due to our choice of $p_t^\thr$ in \eqref{eq:score-estimate} and $c_\rho \geq 2$.
%
By our construction of the score estimator in \eqref{eq:score-estimate}, this implies that for any $x\in\cF_t$, on the event $\cE_t(x)$, we have
\begin{align}
	\wh s_{t}(x)=\frac{\wh g_t(x)}{\wh p_{t}(x)}. \notag
\end{align}

Let us decompose
\begin{align}
& \bE\Big[\big\| \wh{s}_{t}(Z_t)-s_{t}(Z_t) \big\|^2_2\Big] = \int_{\bR^d} \bE\Big[ \big\| \wh{s}_{t}(x)-s_{t}(x) \big\|^2_2 \Big] p_{t}(x) \diff x \notag\\
& \qquad = \underbrace{\int_{\cF_t} \bE\Big[ \big\| \wh{s}_{t}(x)-s_{t}(x) \big\|^2_2 \ind\big\{\cE_t(x)\big\} \Big] p_{t}(x) \diff x}_{\defnrev \chi_1}
+ \underbrace{\int_{\cF_t^\setc} \bE\Big[ \big\| \wh{s}_{t}(x)-s_{t}(x) \big\|^2_2 \ind\big\{\cE_t(x)\big\} \Big] p_{t}(x) \diff x}_{\defnrev \chi_2} \notag\\
& \qquad \quad + \underbrace{\int_{\bR^d} \bE\Big[ \big\| \wh{s}_{t}(x)-s_{t}(x) \big\|^2_2 \ind\big\{\cE_t^\setc(x)\big\} \Big] p_{t}(x) \diff x}_{\defnrev \chi_3}. \label{eq:score-error-temp}
\end{align}

In what follows, we shall bound $\chi_1$, $\chi_2$, and $\chi_3$ individually.

\paragraph*{Bounding $\chi_1$.}
For the term $\chi_1$, we can use \eqref{eq:MSE-score} in Lemma~\ref{lemma:MSE-score-high-density} to derive
\begin{align*}
\chi_1
% &= \int_{\cF_t} \bE\Big[ \big\| \wh{s}_{t}(x)-s_{t}(x) \big\|^2_2 \ind\big\{\wh p_{t}(x) \geq \} \ind\big\{\cE_t(x)\big\} \Big] p_{t}(x) \diff x 
\lesssim \frac1{(2\pi)^{d/2}} \frac{1}{nt^{d/2+1}} |\cF_t| + \frac1{(2\pi)^{d/2}}\frac{1}{nt^{d/2}}  \int_{\cF_t} \|s_{t}(x)\|_2^2 \diff x.
\end{align*}

% By , one has
% \begin{align}
% 	|\cF_t| \lesssim (\sigma^2 + t)^{d/2} \leq 2^{d/2-1} (t^{d/2} + \sigma^d) \label{eq:density-ratio-integral-UB}.
% \end{align}
% In addition, 
% \begin{align}
% 	\int_{\cF_t} \|s_{t}(x)\|_2^2 \diff x
% 	\lesssim
% 	\label{eq:score-l2-norm-integral-UB}
% \end{align}
%
Invoking Lemma~\ref{lemma:high-density-set-bound}, we know from \eqref{eq:high-density-set-UB}--\eqref{eq:high-density-set-score-UB} that
\begin{align}
	\chi_1 &\leq \frac1{(2\pi)^{d/2}} \frac{1}{nt^{d/2+1}} C_5 (t^{d/2} + \sigma^d)(\log n)^{d/2} + \frac1{(2\pi)^{d/2}}\frac{1}{nt^{d/2}} C_5 \frac1t (t^{d/2} + \sigma^d)(\log n)^{d/2+1} \notag \\
	& \leq \frac{2C_5}{(2\pi)^{d/2}}\frac{t^{d/2} + \sigma^d}{nt^{d/2+1}} (\log n)^{d/2+1} \label{eq:score-K1}.
\end{align}


\paragraph*{Bounding $\chi_2$.}

% Recall the definition of $\cF_t^c = \{x\in\bR^d \colon p_{t}(x) < \rho_t \}$ in \eqref{eq:rho-t}.
\begin{align*}
	\chi_2 & \leq \int_{\cF_t^\setc} \bE\Big[ \| \wh{s}_{t}(x)-s_{t}(x) \|^2_2 \Big] p_{t}(x) \diff x \notag\\
	&  = \int_{\cF_t^\setc} \bE\Big[ \| \wh{s}_{t}(x)-s_{t}(x) \|^2_2  \ind\big\{\wh p_{t}(x) < p_t^\thr \big\} \Big] p_{t}(x) \diff x + \int_{\cF_t^\setc} \bE\Big[ \| \wh{s}_{t}(x)-s_{t}(x) \|^2_2 \ind\big\{\wh p_{t}(x) \geq p_t^\thr \big\} \Big] p_{t}(x) \diff x \notag\\
	&  
	\leq \underbrace{\int_{\cF_t^\setc} \|s_{t}(x) \|^2_2 \,p_{t}(x) \diff x}_{\defnrev (\mathrm{I})}+\underbrace{\int_{\cF_t^\setc} \bE\Bigg[ \bigg\| \frac{\wh g_t(x)}{\wh p_{t}(x)}-s_{t}(x) \bigg\|^2_2 \ind\big\{\wh p_{t}(x) \geq p_t^\thr \big\} \Bigg] p_{t}(x) \diff x}_{\defnrev (\mathrm{II})}.
\end{align*}
where the last step holds since $\wh s_{t}(x) = 0$ when $\wh p_{t}(x) < p_t^\thr$ and $\wh s_{t}(x) = \wh g_t(x) / \wh p_{t}(x)$ otherwise.

Regarding the term (I), we can invoke \eqref{eq:prob-small-score} from Lemma~\ref{lemma:prob-small-density} to bound
\begin{align}
	(\mathrm I) \leq C_d \frac{t^{d/2}+\sigma^d}{nt^{d/2+1}} (\log n)^{d/2+2}+ \frac{d^{3/2}}{n^4t} \asymp C_d \frac{t^{d/2}+\sigma^d}{nt^{d/2+1}} (\log n)^{d/2+2}, \label{eq:score-K2-I}
\end{align}
for some constant $C_d >0$ that only depends on $d$, where the last step holds as long as $n\geq d$.


Turning to the term (II), one can decompose 
\begin{align}
	\bigg\|\frac{\wh{g}_t(x)}{\wh{p}_t(x)}- s_{t}(x) \bigg\|_2 &= \bigg\|\frac{\wh{g}_t(x)}{\wh{p}_t(x)}- \frac{g_t(x)}{p_{t}(x)} \bigg\|_2 = \bigg\| \frac{\wh{g}_t(x)-g_t(x)}{\wh{p}_t(x)} + \frac{p_{t}(x)-\wh p_{t}(x)}{\wh p_{t}(x)}\frac{g_t(x)}{p_{t}(x)} \bigg\|_2 \notag \\
	& \leq \frac{1}{\wh{p}_t(x)} \big\|\wh{g}_t(x)-g_t(x)\big\|_2
	+ \frac{1}{\wh{p}_t(x)} \big|\wh{p}_t(x)-p_{t}(x)\big| \|s_{t}(x)\|_2. \label{eq:score-estimate-decomp}
\end{align}
%
Since $\wh p_{t}(x) \geq p_t^\thr$, one has
\begin{align}
	\bigg\| \frac{\wh g_t(x)}{\wh p_{t}(x)}-s_{t}(x) \bigg\|_2 \ind\big\{\wh p_{t}(x) \geq p_t^\thr \big\}
	& \leq \frac{1}{p_t^\thr} \big\|\wh{g}_t(x)-g_t(x)\big\|_2
	+ \frac{1}{p_t^\thr} \big|\wh{p}_t(x)-p_{t}(x)\big| \|s_{t}(x)\|_2. \label{eq:chi-2-temp}
	% \\
	% & \asymp n^2(2\pi t)^{d} \big\|\wh{g}_t(x)-g_t(x)\big\|_2^2
	% + n^2(2\pi t)^{d} \big|\wh{p}_t(x)-p_{t}(x)\big|^2 \|s_{t}(x)\|_2^2, \notag
\end{align}
Thus, the first quantity in \eqref{eq:score-estimate-decomp} can be bounded as
\begin{align*}
	\frac{1}{p^2_\thr} \bE\Big[\big\|\wh{g}_t(x)-g_t(x)\big\|_2^2\Big] 
	& \lesssim  \frac{1}{(p_t^\thr)^2} \frac{1}{(2\pi)^{d/2}}  \frac{p_{t}(x)}{nt^{d/2+1}}  \notag\\
	& \lesssim  \frac{\rho_t}{(p_t^\thr)^2} \frac{1}{(2\pi)^{d/2}}  \frac{1}{nt^{d/2+1}}  \notag\\
	& \asymp \frac{n(2\pi t)^{d/2}}{\log n}\frac{1}{(2\pi)^{d/2}}  \frac{1}{nt^{d/2+1}} \notag\\
	& = \frac{1}{t\log n}
\end{align*}
where (i) uses \eqref{eq:MSE-pdf} in Lemma~\ref{lemma:MSE-density}; (ii)  is true since $p_{t}(x) < \rho_t$ on $\cF_t^\setc$; (ii) follows from our choice of $p_t^\thr$ and $\rho_t$ in \eqref{eq:score-estimate} and \eqref{eq:rho-t}, respectively.

Similarly, we can also use \eqref{eq:MSE-g} in Lemma~\ref{lemma:MSE-density} to control the second term in \eqref{eq:score-estimate-decomp} as
\begin{align*}
	 \frac{1}{(p_t^\thr)^2} \bE\Big[\big|\wh{p}_t(x)-p_{t}(x)\big|^2 \Big]\|s_{t}(x)\|_2^2  & \lesssim  \frac{1}{(p_t^\thr)^2} \frac{1}{(2\pi)^{d/2}}  \frac{p_t}{nt^{d/2}} \|s_{t}(x)\|_2^2  \notag\\
	& \numpf{i}{\leq}  \frac{\rho_t}{(p_t^\thr)^2} \frac{1}{(2\pi)^{d/2}}  \frac{1}{nt^{d/2}} \|s_{t}(x)\|_2^2  \notag \\
	& \numpf{ii}{\lesssim} \frac{\|s_{t}(x)\|_2^2}{\log n},
\end{align*}
Putting the above bounds together shows that
\begin{align}
	\bigg\| \frac{\wh g_t(x)}{\wh p_{t}(x)}-s_{t}(x) \bigg\|_2^2 \ind\big\{\wh p_{t}(x) \geq p_t^\thr \big\} \lesssim \frac{1}{t\log n} + \frac{\|s_{t}(x)\|_2^2}{\log n}, \label{eq:score-K2-II-temp}
\end{align}
which further leads to
\begin{align}
	(\mathrm{II}) \lesssim \frac1{\log n} \int_{\cF_t^\setc} \bigg(\frac{1}{t} + \|s_{t}(x)\|_2^2\bigg)p_{t}(x) \diff x \lesssim \frac{1}{(2\pi)^{d/2}} \frac{t^{d/2}+\sigma^d}{nt^{d/2+1}} (\log n)^{d/2+2}, \label{eq:score-K2-II}
\end{align}
where (i) is true since $p_{t}(x) \leq \rho_t$ on $\cF_t^\setc$; (ii) follows from our choice of $p_t^\thr$ and $\rho_t$ in \eqref{eq:score-estimate} and \eqref{eq:rho-t}, (iii) invokes Lemma~\ref{lemma:prob-small-density} again.

Collecting \eqref{eq:score-K2-I} and \eqref{eq:score-K2-II} together gives that
\begin{align}
	\chi_2 \leq (\mathrm{I}) + (\mathrm{II}) \lesssim \frac{}{} \frac{t^{d/2}+\sigma^d}{nt^{d/2+1}} (\log n)^{d/2+2}. \label{eq:score-K2}
\end{align}
for some constant $C_\score > 0$ that only depends on $d$.


\paragraph*{Bounding $\chi_3$.}
As for the quantity $\chi_3$, applying the Cauchy-Schwartz inequality yields
\begin{align}
& \int_{\bR^d} \bE\Big[ \big\| \wh{s}_{t}(x)-s_{t}(x) \big\|^2_2 \ind\big\{\cE^\setc(x)\big\} \Big] p_{t}(x) \diff x \notag \\
& \qquad \leq \int_{\bR^d} \sqrt{\bE\big[\| \wh{s}_{t}(x)-s_{t}(x)\|^4_2 \big]} \sqrt{\bP\big(\cE^\setc(x)\big)}\, p_{t}(x) \diff x \notag\\
& \qquad \lesssim n^{-5} \int_{\bR^d} \Big(\sqrt{\bE\big[\| \wh{s}_{t}(x)\|_2^4 \big]} + \|s_{t}(x) \|^2_2\Big)\, p_{t}(x) \diff x
\end{align}
where the last step uses \eqref{eq:density-concen-ineq} and $\sqrt{a+b}\leq \sqrt{a}+\sqrt{b}$ for any $a,b\geq 0$.


By our choice of $\wh{s}_{t}(x)$ in \eqref{eq:score-estimate}, we have
\begin{align*}
	\big\| \wh{s}_{t}(x)\big\|_2 &= \frac{1}{\wh{p}_t(x)}\|  \wh g_t(x)\|_2 \ind\big\{\wh{p}_t(x) \geq p_t^\thr\big\} \leq \frac1{p_t^\thr} \big\| \wh{g}_t(x)\big\|_2.
\end{align*}
%
Recalling the expression of $\wh g_t(x)$ in \eqref{eq:g-hat}, one can bound
\begin{align}
	\big\| \wh{g}_t(x)\big\|_2
	& = \bigg\| \frac1{nt}\sum_{i=1}^n (X_i-x)\vphi_t(X_i-x)\bigg\|_2 \notag\\
	& \leq \max_{i\in[n]}\frac1{t} \big\| (X_i-x)\vphi_t(X_i-x)\big\|_2 \notag\\
	& \leq \frac1t \sup_{x\in\bR^d}\bigg\{\|x\|_2 \frac1{(2\pi t)^{d/2}}\exp\left(-\|x\|_2^2/\left(2t\right)\right)\bigg\} \notag\\
	& = \frac1{\sqrt{e}\,(2\pi)^{d/2}}\frac1{t^{(d+1)/2}}. \label{eq:g-hat-UB}
\end{align}
%
Plugging the value of $p_t^\thr$ in \eqref{eq:score-estimate} into \eqref{eq:g-hat-UB} gives
\begin{align}
	\| \wh{s}_{t}(x)\|_2 \leq \frac1{p_t^\thr} \big\| \wh{g}_t(x)\big\|_2 \lesssim \frac{n(2\pi t)^{d/2}}{\log n} \frac1{(2\pi)^{d/2}}\frac1{t^{(d+1)/2}} \leq \frac{n}{\sqrt t},
\end{align}
thereby leading to
\begin{align}
	\int_{\bR^d} \sqrt{\bE\big[ \| \wh{s}_{t}(x)\|_2^4\big]}\,p_{t}(x) \diff x 
	& \lesssim  \frac{n^2}{t}. \label{eq:score-K3-I}
\end{align}

Additionally, applying \eqref{eq:score-lp-norm} from Lemma~\ref{lemma:score-lp-norm} gives
\begin{align}
	\int_{\bR^d} \|s_{t}(x)\|^2_2\,p_{t}(x) \diff x
	\lesssim \frac{d}{t}, \label{eq:score-K3-II}
\end{align}

Therefore, combining \eqref{eq:score-K3-I} and \eqref{eq:score-K3-II} reveals that
\begin{align}
\chi_3 \lesssim \frac{d}{n^5t} + \frac{1}{n^3t} \asymp \frac{1}{n t}
	\label{eq:score-K3}.
\end{align}
where the last step holds as long as $n \geq d$.

\paragraph*{Putting bounds for $\chi_1,\chi_2,\chi_3$ together.}

To finish up, substituting \eqref{eq:score-K1}, \eqref{eq:score-K2}, and \eqref{eq:score-K3} into \eqref{eq:score-error-temp} yields
\begin{align*}
	\int_{\bR^d} \bE\Big[ \big\| \wh{s}_{t}(x)-s_{t}(x) \big\|^2_2 \Big] p_{t}(x) \diff x &\leq \chi_1 +\chi_2 +\chi_3 \leq C_\score\bigg( \frac1{nt} + \frac{\sigma^d}{nt^{d/2+1}} \bigg)(\log n)^{d/2+2}
\end{align*}
for some constant $C_\score = C_\score(d)>0$  that only depends on $d$. This concludes the proof of Theorem~\ref{thm:score-error}.

As for the .
\begin{align*}
	\bE\Big[\big\|\wh s_t^\sm(Z_t)-s_t(Z_t)\big\|_2^2\Big]\leq \bE\Big[\big\|\wh s_t^\sm(Z_t)-\wh s_t(Z_t)\big\|_2^2\Big] + \bE\Big[\big\|\wh s_t(Z_t)-s_t(Z_t)\big\|_2^2\Big]
\end{align*}

\begin{align*}
	\big\|(\wh s_t \ast \vphi_\delta)(x)-\wh s_t(x)\big\|_2^2 &= \bigg\|\int_{\bR^d}\big(\wh s_t(y)-\wh s_t(x)\big) \vphi_\delta(x-y) \diff y\bigg\|_2^2 \\
	&\leq \int_{\bR^d} \big\|\wh s_t(y)-\wh s_t(x)\big\|_2^2 \vphi_\delta(x-y) \diff y
\end{align*}

\begin{align*}
	\bE\Big[\big\|\wh s_t^\sm(Z_t)-\wh s_t(Z_t)\big\|_2^2\Big] &= \int_{\bR^d}\big\|\wh s_t^\sm(x)-\wh s_t(x)\big\|_2^2\,p_t(x) \diff x \\
	& = \int_{\bR^d}\big\|(\wh s_t \ast \vphi_\delta)(x)-\wh s_t(x)\big\|_2^2\,p_t(x) \diff x \\
	& \leq \int_{\bR^d}\int_{\bR^d} \big\|\wh s_t(y)-\wh s_t(x)\big\|_2^2 \vphi_\delta(x-y) \diff y \,p_t(x) \diff x 
\end{align*}



\subsection{Proof of Theorem~\ref{thm:Jacobian-error}}\label{sub:proof_of_lemma_ref_lemma_Jacobian-error}

Similar to the proof of Theorem~\ref{thm:score-error} in Appendix~\ref{sub:proof_of_lemma_ref_lemma_score-error}, we can decompose
\begin{align}
& \int_{\bR^d} \bE\Big[ \big\| J_{\wh{s}_t}(x)-J_{s_{t}}(x) \big\| \Big] p_{t}(x) \diff x \notag\\
& \qquad = \underbrace{\int_{\cF_t} \bE\Big[ \big\| J_{\wh{s}_t}(x)-J_{s_{t}}(x) \big\| \ind\big\{\cE_t(x)\big\} \Big] p_{t}(x) \diff x}_{\defn \xi_1}
+ \underbrace{\int_{\cF_t^\setc} \bE\Big[ \big\| J_{\wh{s}_t}(x)-J_{s_{t}}(x) \big\| \ind\big\{\cE_t(x)\big\} \Big] p_{t}(x) \diff x}_{\defn \xi_2} \notag\\
& \qquad \quad + \underbrace{\int_{\bR^d} \bE\Big[ \big\| J_{\wh{s}_t}(x)-J_{s_{t}}(x) \big\| \ind\big\{\cE_t^\setc(x)\big\} \Big] p_{t}(x) \diff x}_{\defn \xi_3}. \label{eq:Jacobian-error-temp}
\end{align}
It suffices to control these three quantities individually.

\paragraph*{Bounding $\xi_1$.}
Applying \eqref{eq:MSE-Jacobian}, we have
\begin{align}
	% & \int_{\cF_t} \bE\Big[ \big\| J_{\wh{s}_t}(x)-J_{s_{t}}(x) \big\| \ind\big\{\cE_t(x)\big\} \Big] p_{t}(x) \diff x \notag\\
	\xi_1& \lesssim \frac{|\cF_t|}{nt^{d/2+1}}  + \frac{\log n}{\sqrt{n}\,t^{d/4+1}} \int_{\cF_t}  \sqrt{p_{t}(x)} \diff x + \frac{1}{nt^{d/2}} \int_{\cF_t}  \|s_{t}(x)\|_2^2 \diff x + \frac{1}{\sqrt{n}t^{d/4}} \int_{\cF_t}  \sqrt{p_{t}(x)} \|s_{t}(x)\|_2^2 \diff x. \label{eq:Jacobian-error-temp-term1}
\end{align}

From \eqref{eq:high-density-set-UB} in Lemma~\ref{lemma:high-density-set-bound}, it is easily seen that
\begin{align}
	\frac{|\cF_t|}{nt^{d/2+1}}  \leq C_5 \frac{t^{d/2}+\sigma^d}{nt^{d/2+1}} (\log n)^{d/2} \label{eq:Jacobian-error-term1}.
\end{align}
%
In addition,
\begin{align}
	\frac{\log n}{\sqrt{n}\,t^{d/4+1}}\int_{\cF_t}  \sqrt{p_{t}(x)} \diff x 
	& \numpf{i}{\leq} \frac{\log n}{\sqrt{n}\,t^{d/4+1}}\bigg(\int_{\cF_t} p_{t}(x) \diff x\bigg)^{1/2} \sqrt{|\cF_t|} \leq \frac{\log n}{\sqrt{n}\,t^{d/4+1}} \sqrt{|\cF_t|} \notag\\
	& \numpf{ii}{\leq} C_5\frac{t^{d/4}+\sigma^{d/2}}{\sqrt{n}\,t^{d/4+1}} (\log n)^{d/4+1} \label{eq:Jacobian-error-term2}.
\end{align}
where (i) uses the Cauchy-Schwartz inequality, (ii) applies \eqref{eq:high-density-set-UB} in Lemma~\ref{lemma:high-density-set-bound} again.
%
Also, by \eqref{eq:high-density-set-score-UB} in Lemma~\ref{lemma:high-density-set-bound}, the third term is upper bounded by
\begin{align}
	\frac{1}{nt^{d/2}} \int_{\cF_t}  \|s_{t}(x)\|_2^2 \diff x \leq C_5 \frac{t^{d/2}+\sigma^d}{nt^{d/2+1}}(\log n)^{d/2+1} \label{eq:Jacobian-error-term3}.
\end{align}
%
Finally, 
% \begin{align}
% 	\frac{1}{\sqrt{n}t^{d/4}}\int_{\cF_t}  \sqrt{p_{t}(x)} \|s_{t}(x)\|_2^2 \diff x & \numpf{i}{\leq} \frac{1}{\sqrt{n}t^{d/4}}\bigg(\int_{\cF_t}  p_{t}(x) \diff x\bigg)^{1/2}\bigg(\int_{\cF_t}  \|s_{t}(x)\|_2^4 \diff x\bigg)^{1/2} \notag\\
% 	& \numpf{iii}{\leq} \sqrt{C_5} \frac{t^{d/4}+\sigma^{d/2}}{\sqrt{n}t^{d/4+1}} (\log n)^{d/4+1}. \label{eq:Jacobian-error-term4}
% \end{align}
\begin{align}
	\frac{1}{\sqrt{n}t^{d/4}}\int_{\cF_t}  \sqrt{p_{t}(x)} \|s_{t}(x)\|_2^2 \diff x & \numpf{i}{\leq} \frac{1}{\sqrt{n}t^{d/4}}\bigg(\int_{\cF_t} p_{t}(x) \|s_{t}(x)\|_2^4 \diff x\bigg)^{1/2} \sqrt{|\cF_t|} \notag\\
	& \numpf{ii}{\leq} \frac{1}{\sqrt{n}t^{d/4}}\frac dt \sqrt{C_5}\big((t+\sigma^2)\log n\big)^{d/4} \notag\\
	& \numpf{iii}{\leq} \sqrt{C_5} \frac{t^{d/4}+\sigma^{d/2}}{\sqrt{n}t^{d/4+1}} (\log n)^{d/4}. \label{eq:Jacobian-error-term4}
\end{align}
Here, (i) uses the Cauchy-Schwartz inequality; (ii) applies \eqref{eq:high-density-set-score-UB} in Lemma~\ref{lemma:high-density-set-bound}.

Substituting \eqref{eq:Jacobian-error-term1}--\eqref{eq:Jacobian-error-term4} into \eqref{eq:Jacobian-error-temp-term1} results in
\begin{align}
	\xi_1 &\lesssim \bigg(\frac{1}{nt} + \frac{\sigma^d}{nt^{d/2+1}}\bigg)(\log n)^{d/2+1} + \bigg(\frac{1}{\sqrt{n}\,t} + \frac{\sigma^{d/2}}{\sqrt{n}\,t^{d/4+1}}\bigg)(\log n)^{d/4+1} \notag\\
	& \lesssim  \bigg(\frac{1}{\sqrt{n}\,t} + \frac{\sigma^{d/2}}{\sqrt{n}\,t^{d/4+1}} + \frac{\sigma^d}{nt^{d/2+1}}\bigg)(\log n)^{d/2+1}  \label{eq:Jacobian-K1}.
\end{align}


\paragraph*{Bounding $\xi_2$.}
Recall that for any $x\in\cF_t^c $, one has $p_{t}(x) < \rho_t$.
\begin{align*}
	\xi_2 & \leq \int_{\cF_t^\setc} \bE\Big[ \| J_{\wh{s}_t}(x)-J_{s_{t}}(x) \| \Big] p_{t}(x) \diff x \notag\\
	&  = \int_{\cF_t^\setc} \bE\Big[ \| J_{\wh{s}_t}(x)-J_{s_{t}}(x) \|  \ind\big\{\wh p_{t}(x) < p_t^\thr \big\} \Big] p_{t}(x) \diff x + \int_{\cF_t^\setc} \bE\Big[ \| J_{\wh{s}_t}(x)-J_{s_{t}}(x) \| \ind\big\{\wh p_{t}(x) \geq p_t^\thr \big\} \Big] p_{t}(x) \diff x \notag\\
	&  
	\leq \underbrace{\int_{\cF_t^\setc} \|J_{s_{t}}(x) \| \,p_{t}(x) \diff x}_{\defnrev (\mathrm{I})}+\underbrace{\int_{\cF_t^\setc} \bE\Big[ \| J_{\wh{s}_t}(x)-J_{s_{t}}(x) \| \ind\big\{\wh p_{t}(x) \geq p_t^\thr \big\} \Big] p_{t}(x) \diff x}_{\defnrev (\mathrm{II})}.
\end{align*}
where the last step holds since $J_{\wh s_{t}(x)} = 0$ when $\wh p_{t}(x) < p_t^\thr$.

To bound the term (I), we can use Lemma~\ref{lemma:prob-small-density} to obtain
\begin{align}
	(\mathrm I) \leq C_d \frac{t^{d/2}+\sigma^d}{nt^{d/2+1}} (\log n)^{d/2+2}+ \frac{d^{3/2}}{n^4t} \asymp C_d \frac{t^{d/2}+\sigma^d}{nt^{d/2+1}} (\log n)^{d/2+2}, \label{eq:Jacobian-K2-I}
\end{align}
for some constant $C_d >0$ that only depends on $d$, where the last step holds as long as $n\geq d$.


As for the term (II), on the event $\big\{\wh p_{t}(x) \geq p_t^\thr\big\}$, we can use \eqref{eq:error-Jacobian} to derive
\begin{align*}
& \big\|J_{\wh{s}_t}(x)-J_{s_{t}}(x) \big\| \ind\big\{\wh p_{t}(x) \geq p_t^\thr \big\} \notag\\
& \qquad \leq 
	\bigg(\frac{\|\wh{H}_t(x)-H_t(x)\|}{\wh{p}_t(x)}
	+ \frac{|\wh p_{t}(x)-p_{t}(x)|}{\wh p_{t}(x)}\frac{\|H_t(x)\|}{p_{t}(x)}
	+ \bigg\| \frac{\wh g_t(x)}{\wh p_{t}(x)}+s_{t}(x) \bigg\|_2\bigg\| \frac{\wh g_t(x)}{\wh p_{t}(x)}-s_{t}(x) \bigg\|_2\bigg) \ind\big\{\wh p_{t}(x) \geq p_t^\thr \big\} \\
& \qquad \lesssim \frac{\|\wh{H}_t(x)-H_t(x)\|}{p_t^\thr}
	+ \frac{|\wh p_{t}(x)-p_{t}(x)|}{p_t^\thr}\frac{\|H_t(x)\|}{p_{t}(x)}
	+ \frac{\|\wh g_t(x)\|_2^2}{(p_t^\thr)^2}+\|s_{t}(x)\|_2^2 + \bigg\| \frac{\wh g_t(x)}{\wh p_{t}(x)}-s_{t}(x) \bigg\|_2^2\ind\big\{\wh p_{t}(x) \geq p_t^\thr \big\}
\end{align*}
where the last step uses the triangle inequality and AM-GM inequality. Hence, it suffices to control these quantities separately.
\begin{itemize}
	\item For any $x\in\cF_t^\setc$, one has
	\begin{align}
		\frac{1}{p_t^\thr}\bE\Big[\big\|\wh{H}_t(x)-H_t(x)\big\|\Big]
		&\numpf{i}{\lesssim} \frac1{p_t^\thr} \bigg(\frac1{(2\pi)^{d/2}}\frac1{nt^{d/2+1}} + \frac1{(2\pi)^{d/4}} \frac{\sqrt{p_{t}(x)}}{\sqrt{n}\,t^{d/4+1}}\bigg) \notag\\
		&\numpf{ii}{\leq} \frac1{p_t^\thr} \bigg(\frac1{(2\pi)^{d/2}}\frac1{nt^{d/2+1}} + \frac1{(2\pi)^{d/4}} \frac{\sqrt{\rho_t}}{\sqrt{n}\,t^{d/4+1}}\bigg) \notag\\
		&\numpf{iii}{\lesssim}\frac{n(2\pi t)^{d/2}}{\log n} \bigg(\frac1{(2\pi)^{d/2}}\frac1{nt^{d/2+1}} + \sqrt{\frac{\log n}{n(2\pi t)^{d/2}}}\frac1{(2\pi)^{d/4}} \frac{1}{\sqrt{n}\,t^{d/4+1}}\bigg) \notag\\
		& \asymp \frac1{t\sqrt{\log n}} \label{eq:chi-term1}
	\end{align}
	where (i) uses \eqref{eq:Phi-error-exp-UB} in Lemma~\ref{lemma:MSE-density}; (ii) $p_{t}(x)\leq \rho_t$ on the set $\cF_t^\setc$; (iii) plugs in the values of $p_t^\thr$ and $\rho_t$
	\item Similarly, we can  to get
	\begin{align}
	\frac{\bE\big[|\wh p_{t}(x)-p_{t}(x)|\big]}{p_t^\thr}\frac{\|H_t(x)\|}{p_{t}(x)}
	& \numpf{i}{\leq} \frac{\sqrt{\bE\big[|\wh p_{t}(x)-p_{t}(x)|^2\big]}}{p_t^\thr}\frac{\|H_t(x)\|}{p_{t}(x)} \notag\\
	& \numpf{ii}{\lesssim} \frac{1}{p_t^\thr}\sqrt{\frac{p_{t}(x)}{n(2\pi t)^{d/2}}}\frac{\|H_t(x)\|}{p_{t}(x)} \notag\\
	& \numpf{iii}{\leq} \frac{1}{p_t^\thr}\sqrt{\frac{\rho_t}{n(2\pi t)^{d/2}}}\frac{\|H_t(x)\|}{p_{t}(x)} \notag\\
	& \numpf{iv}{\lesssim} \sqrt{\frac{n(2\pi t)^{d/2}}{\log n}}\sqrt{\frac{1}{n(2\pi t)^{d/2}}}\frac{\|H_t(x)\|}{p_{t}(x)} \notag\\
	& = \frac1{\sqrt{\log n}}\frac{\|H_t(x)\|}{p_{t}(x)} \label{eq:chi-term2}
	\end{align}
where (i) uses the Cauchy-Schwartz inequality; (ii) arises from \eqref{eq:MSE-pdf} in Lemma~\ref{lemma:MSE-density}; (iii) holds as $p_{t}(x)\leq \rho_t$ on the set $\cF_t^\setc$; (iv) is due the choices of $p_t^\thr$ and $\rho_t$.

\item By \eqref{eq:MSE-g} in Lemma~\ref{lemma:MSE-density}, one knows that on the set $\cF_t^\setc$,
\begin{align}
	\frac1{(p_t^\thr)^2}\bE\Big[\big\|\wh g_t(x)\big\|_2^2\Big] 
	&\numpf{i}{\lesssim} \frac1{(p_t^\thr)^2} \bE\Big[\big\|\wh g_t(x)-g_t(x)\big\|_2^2\Big] + \frac1{(p_t^\thr)^2}\big\|g_t(x)\big\|_2^2 \notag\\
	& \numpf{ii}{\leq} \frac1{(p_t^\thr)^2} \frac1{(2\pi)^{d/2}} \frac{p_{t}(x)}{nt^{d/2+1}} + \frac{p_t^2(x)}{(p_t^\thr)^2}  \|s_{t}(x)\|_2^2, \notag\\
	& \numpf{iii}{\leq} \frac1{(p_t^\thr)^2} \frac1{(2\pi)^{d/2}} \frac{\rho_t}{nt^{d/2+1}} + \frac{\rho_t^2}{(p_t^\thr)^2}  \|s_{t}(x)\|_2^2 \notag\\
	& \numpf{iv}{\asymp} \frac{n(2\pi t)^{d/2}}{\log n} \frac1{(2\pi)^{d/2}} \frac{1}{nt^{d/2+1}} + \|s_{t}(x)\|_2^2 \notag\\
	& =  \frac{1}{t\log n}+ \|s_{t}(x)\|_2^2 \label{eq:chi-term3}
\end{align}
where (i) applies the AM-GM inequality; (ii) invokes \eqref{eq:MSE-pdf} in Lemma~\ref{lemma:MSE-density}; (iii) holds as $p_{t}(x)\leq \rho_t$ on the set $\cF_t^\setc$; (iv) is due the choices of $p_t^\thr$ and $\rho_t$.

\item The last term has been controlled in \eqref{eq:score-K2-II-temp}.


\item Combining \eqref{eq:chi-term1}--\eqref{eq:chi-term3} with \eqref{eq:score-K2-II-temp}, we find that
\begin{align}
	(\mathrm{II}) & \lesssim \int_{\cF_t^\setc} \bigg(\frac1{\sqrt{\log n}}\frac{\|H_t(x)\|}{p_{t}(x)} + \frac{1}{t\sqrt{\log n}} + \|s_{t}(x)\|_2^2 \bigg) p_{t}(x)\diff x \lesssim \frac{1}{(2\pi)^{d/2}} \frac{t^{d/2}+\sigma^d}{nt^{d/2+1}}, \label{eq:Jacobian-K2-II}
\end{align}
\end{itemize}

Collecting \eqref{eq:Jacobian-K2-I} and \eqref{eq:Jacobian-K2-II} together gives that
\begin{align}
	\xi_2 \leq (\mathrm{I}) + (\mathrm{II}) \lesssim \frac{t^{d/2}+\sigma^d}{nt^{d/2+1}}(\log n)^{d/2+2}. \label{eq:Jacobian-K2}
\end{align}



\paragraph*{Bounding $\xi_3$.}
It remains to control the quantity $\xi_3$. We can first use the Cauchy-Schwartz inequality to bound
\begin{align}
% & \int_{\bR^d} \bE\Big[ \big\| J_{\wh{s}_t}(x)-J_{s_{t}}(x) \big\| \ind\big\{\cE^\setc(x)\big\} \Big] p_{t}(x) \diff x \notag \\
\xi_3 & \leq \int_{\bR^d} \sqrt{\bE\Big[ \big\| J_{\wh{s}_t}(x)-J_{s_{t}}(x) \big\|^2 \Big]} \sqrt{\bP\big(\cE^\setc(x)\big)}\, p_{t}(x) \diff x \notag\\
& \lesssim n^{-5} \int_{\bR^d} \Big(\sqrt{\bE\Big[ \big\| J_{\wh{s}_t}(x)\big\|^2}\Big] + \|J_{s_{t}}(x) \|\Big)\, p_{t}(x) \diff x,
\end{align}
where the last step uses \eqref{eq:density-concen-ineq}, the AM-GM inequality, and $\sqrt{a+b}\leq \sqrt{a}+\sqrt{b}$ for any $a,b\geq 0$.


By the expression of $J_{\wh{s}_t}(x)$ in \eqref{eq:Jacobian-score-est-expression}, we can bound
\begin{align*}
	\big\| J_{\wh{s}_t}(x)\big\| &\leq \left\| -\frac1t I_d + \frac{1}{\wh{p}_t(x)}\wh{H}_t(x) - \frac{1}{\wh{p}_t^2(x)}\wh{g}_t(x)\wh{g}_t(x)^\top \right\| \ind\big\{\wh{p}_t(x) \geq p_t^\thr\big\} \\
	& \lesssim \frac1{t} + \frac{1}{p_t^\thr}\big\|\wh{H}_t(x)\big\| + \frac1{(p_t^\thr)^2} \big\| \wh{g}_t(x)\big\|_2^2 \\
	& \numpf{i}{\lesssim} \frac1t + \frac{1}{p_t^\thr} \frac{1}{(2\pi)^{d/2}} \frac{1}{t^{d/2+1}} + \frac{1}{(p_t^\thr)^2} \frac1{(2\pi)^{d}}\frac1{t^{(d+1)}} \\
	& \numpf{ii}{\asymp} \frac1t + \frac{n(2\pi t)^{d/2}}{\log n} \frac{1}{(2\pi)^{d/2}} \frac{1}{t^{d/2+1}} + \frac{n^2(2\pi t)^{d}}{\log^2 n} \frac1{(2\pi)^{d}}\frac1{t^{(d+1)}} \\
	& \asymp \frac{n^2}{\log^2n}\frac1t,
\end{align*}
where (i) uses \eqref{eq:Sigma-hat-UB} and \eqref{eq:g-hat-UB}; (ii) arises from the choice of $p_t^\thr$ in \eqref{eq:score-estimate}. Hence, we find that
\begin{align}
	\int_{\bR^d} \sqrt{\bE\Big[\big\| J_{\wh{s}_t}(x)\big\|^2\Big]}\,p_{t}(x) \diff x 
	& \lesssim \frac{n^2}{t}. \label{eq:Jacobian-K3-I}
\end{align}

Additionally, by \eqref{eq:Jacobian-lp-norm} in Lemma~\ref{lemma:score-lp-norm}, one has
\begin{align}
	\int_{\bR^d} \big\|J_{s_{t}}(x)\big\|\,p_{t}(x) \diff x
	\lesssim \frac{d}{t}, \label{eq:Jacobian-K3-II}
\end{align}
%
Consequently, putting \eqref{eq:Jacobian-K3-I} and \eqref{eq:Jacobian-K3-II} collectively gives
\begin{align}
\xi_3 \lesssim \frac{d}{n^5t} + \frac{1}{n^3t} \lesssim \frac{1}{n t}
	\label{eq:Jacobian-K3}
\end{align}
where the last inequality is true since $n \geq d$.



\paragraph*{Combining bounds for $\xi_1,\xi_2,\xi_3$ together.}

Plugging \eqref{eq:Jacobian-K1}, \eqref{eq:Jacobian-K2}, and \eqref{eq:Jacobian-K3} into \eqref{eq:Jacobian-error-temp} leads to
\begin{align*}
	\int_{\bR^d} \bE\Big[ \big\| J_{\wh{s}_t}(x)-J_{s_{t}}(x) \big\| \Big] p_{t}(x) \diff x &\leq \xi_1 + \xi_2 + \xi_3 \lesssim  \bigg(\frac{1}{\sqrt{n}\,t} + \frac{\sigma^{d/2}}{\sqrt{n}\,t^{d/4+1}} + \frac{\sigma^d}{nt^{d/2+1}} + \frac{1}{nt} \bigg) (\log n)^{d/2+2} \\
	& \leq C_\jcb \bigg(\frac{1}{\sqrt{n}\,t} + \frac{\sigma^{d/2}}{\sqrt{n}\,t^{d/4+1}} + \frac{\sigma^d}{nt^{d/2+1}} \bigg)(\log n)^{d/2+2}
\end{align*}
for some constant $C_\jcb=C_\jcb(d)>0$ that only depends on $d$.
This finishes the proof of Theorem~\ref{lemma:MSE-Jacobian-high-density}.


